ImGCL: Revisiting Graph Contrastive Learning on Imbalanced Node Classification

Graph contrastive learning (GCL) has attracted a surge of attention due to its superior performance for learning node/graph representations without labels. However, in practice, the underlying class distribution of unlabeled nodes for the given graph is usually imbalanced. This highly imbalanced class distribution inevitably deteriorates the quality of learned node representations in GCL. Indeed, we empirically find that most state-of-the-art GCL methods cannot obtain discriminative representations and exhibit poor performance on imbalanced node classification. Motivated by this observation, we propose a principled GCL framework on Imbalanced node classification (ImGCL), which automatically and adaptively balances the representations learned from GCL without labels. Specifically, we first introduce the online clustering based progressively balanced sampling (PBS) method with theoretical rationale, which balances the training sets based on pseudo-labels obtained from learned representations in GCL. We then develop the node centrality based PBS method to better preserve the intrinsic structure of graphs, by upweighting the important nodes of the given graph. Extensive experiments on multiple imbalanced graph datasets and imbalanced settings demonstrate the effectiveness of our proposed framework, which significantly improves the performance of the recent state-of-the-art GCL methods. Further experimental ablations and analyses show that the ImGCL framework consistently improves the representation quality of nodes in under-represented (tail) classes.

==> 2-Related_work.tex <==
\section{Related work}
\label{sec:related}
% In this section, we proceed by reviewing relevant threads of research including graph contrastive learning and imbalanced learning.
\noindent \textbf{Graph Contrastive Learning.} 
Some recent remarkable progress has been made to adapt contrastive learning methods to the graph domain. Typically, the main idea behind graph contrastive learning~(GCL) is to learn effective representations in which similar sample pairs stay close to each other while dissimilar ones are far apart~\cite{zhu2021empirical}. According to~\cite{tao2021exploring}, we can divide GCL methods into three categories: (1) \emph{contrastive learning} methods~\cite{velivckovic2018deep, sun2019infograph, hassani2020contrastive, you2020graph, zhu2020graph} aim to reduce the distance between two augmented views of the same nodes/graphs~(positive samples), and push apart views of different nodes/graphs~(negative samples). These methods mainly differ in several design choices including graph data augmentations, contrasting modes, and contrastive objectives. DGI~\cite{velivckovic2018deep} adopts the InfoNCE principle~\cite{poole2019variational} to the node classification task by contrasting the node- and graph-level representations of the given graph. InfoGraph~\cite{sun2019infograph} mainly focus on graph classification task by contrasting graph representation of different granularity via mutual information maximization. MVGRL~\cite{hassani2020contrastive} utilizes the graph diffusion matrix to construct the augmentation views of the original graph and then contrast node- and graph-level representation by scoring the agreement between representations. GraphCL~\cite{you2020graph} adopts the SimCLR~\cite{chen2020simpleframework} framework and propose four practical graph augmentation methods to obtain better graph representations. GRACE~\cite{zhu2020graph} capitalizes on the idea that data augmentations for GCL should preserve the property of graphs to highlight important node features.
(2) Negative samples play an important role in contrastive learning methods. However, \emph{asymmetric network} methods~\cite{thakoor2021bootstrapped} get rid of negative samples via the introduction of a predictor network and the stop-gradient operation to avoid mode collapse.
(3) \emph{Feature decorrelation} methods~\cite{zhang2021canonical, bielak2021graph} has recently been introduced as a new solution to GCL. They focus on reducing the redundancy among feature dimensions by introducing a loss function calculated by the cross-correlation matrix of two augmentation views.
Different from our work, these methods mainly assume that the unlabeled graph data distribution is always balanced for GCL. However, in practice, the (unlabeled) class distribution could be highly skewed and lead to sub-optimal generalization on the imbalanced graph dataset.

\noindent \textbf{Imbalanced Learning.} 
% It is well known that the degree of many large graphs follows a scale-free power-law distribution, which is long-tailed and highly imbalanced~\cite{barabasi1999emergence}. 
In this work, we focus on the imbalanced class distribution, which is also ubiquitous for graph datasets. There exists some recent work to study the class imbalance of semi-supervised node classification problems. They mainly improve the imbalanced classification performance by re-balancing the sample ratio of head and tail classes~\cite{zhao2021graphsmote, qu2021imgagn, chawla2002smote} and transfer knowledge from head classes to enhance model performance on tail classes~\cite{liu2020towards, wang2021distance, shi2020multi}. GraphSMOTE~\cite{zhao2021graphsmote} utilizes the SMOTE synthetic over-sampling algorithm to up-sample the tail nodes and then improve their prediction performance. ImGAGN~\cite{qu2021imgagn} aims to improve the representation learning of tail nodes by generating adversarial tail nodes to balance the class distribution of the original graph. DPGNN~\cite{wang2021distance} borrows the idea of metric learning to transfer knowledge from head classes to tail classes to boost model performance. However, they mainly ignore that open-world unlabeled data usually follows the imbalanced distribution, which will lead to performance degradation under unsupervised or self-supervised learning. To our best knowledge, we are the first to explore contrastive learning on \emph{highly} imbalanced graph datasets.



==> Methods.tex <==
\section{Locality-Aware Attention and Adaptive Refined Labeling}
\label{sec:method}

In this section, we propose our LARA
% (\underline{L}ocality-Aware \underline{A}ttention and Adaptive \underline{R}efined L\underline{a}beling) 
framework, which is composed of the following two main components in order---\textbf{locality-aware attention} (Sec. \ref{sec:attention}) and \textbf{adaptive refined labeling} (Sec. \ref{sec:bi-level}), shown in Fig. \ref{fig:framework}. The key idea is that \emph{locality-aware attention} can extract the samples with high $p_x$ and \emph{adaptive refined labeling} can reset the labels of \emph{noisy samples} to boost the performance of predictors. 

\subsection{Locality-Aware Attention}
\label{sec:attention}
\subsubsection{Localization Module}
\ 
\newline
\indent Recalling that $y_{|x} \sim Ber(p_x)$, it is hard to recover Bernoulli's distribution $Ber(p_x)$ from the dataset, as we can only observe one single instance of label $y_{|x}$. Suppose the probability parameter $p_x$ that determines each distribution is continuous with respect to $x$. 
% Then technically, 
We design a \emph{localization module} attending to other observed labels in the dataset to obtain an approximate estimation $\hat{p}_x$ of $p_x$. In the light of the concepts of attention mechanism \cite{vaswani2017attention}, let $\left(x_i, y_i\right)$ denote the key-value pair and $x$ be the query sample processed by the \emph{metric learning module}~(introduced in Sec.~\ref{sec:metric}). The \emph{localization module} can be formulated as follows:
\begin{equation}
    \label{eq:label-attention}
    \hat{p}_x = \sum_{1 \leq i \leq N} y_i \frac{k(x_i, x)}{\sum_{1 \leq j \leq N} k(x_j, x)} \quad,
\end{equation}
where $N$ is the size of the training set, $k(x_i, x)$ is the attention weight \textit{(importance)} between $x$ and $x_i$, and the label of $x_i$ is $y_i$. 
However, in the most general attention mechanisms, the model allows every sample to attend to every other sample.
% , \textcolor{blue}{\sout{\emph{diluting the local information of labels}.}} \textcolor{red}{timeconsuming and immersed in lots of useless information}
Intuitively, closer neighbors of a query point have greater similarity than neighbors which are further away.
We inject the locality structure into the scheme by performing \textit{masked attention} and merely pay attention to the neighbors of $x$, \emph{i.e.,} $\{z: z \in \mathcal{N}(x) \}$. Then we reformulate the \emph{localization module} as follows:
\begin{equation}
    \label{eq:label-attention-reformulate}
    \hat{p}_x = \sum_{z\in \mathcal{N}(x)} y_z \frac{k(z, x)}{\sum_{z \in \mathcal{N}(x)} k(z, x)} \quad.
\end{equation}
% \textcolor{red}{\sout{In Eq. \eqref{eq:attention-weight}, we give two kinds of attention weight that can be applied to the localization module} 
% where $y_z$ denotes the label of instance $z$. 
Furthermore, there exist several reasonable metrics for the implementation of the attention weight in \eqref{eq:label-attention-reformulate}. We recommend two natural approaches: the first is the identical weight and the second is the reciprocal of Euclidean distance $d(z, x)$ considering the influence of distance, detailed as below:
\begin{equation}
    \label{eq:attention-weight}
    % k(z,x) =& 1 \\
    % k(z,x) =& 1/d(z, x) 
    k(z,x) := \left\{
    \begin{array}{lll}
         k_i&= 1  &, \text{ the identical weight}\\
         k_r&= 1/d(z, x) &, \text{ the reciprocal of distance}
    \end{array}
    \right.
\end{equation}
In addition, to obtain the neighbors in the \emph{localization module}, we propose two practical paradigms (detailed in Sec. \ref{sec:implementation}): first, to search the k-nearest neighbors of the query point (K-Neighbor); second, to search the k-nearest neighbors in a given fixed radius (R-Neighbor).

Specifically, in the training phase, we first extract the samples with high $p_x$ satisfying $\hat{p}_x > thres$ in \emph{\underline{l}ocality-aware \underline{a}ttention}~(LA-Attention), which implicitly represent the potentially profitable samples. 
% we then further refine them, that is, train a classifier on the extracted samples to get a more accurate classifier.
% In addition, 
Then we train the more robust model on these selected samples according to the corresponding supervised loss. In the testing phase, we first gather the samples with high $p_x$ by the $\hat{p}_x > thres$ criterion, and then we only make predictions on these selected samples.
Through empirical observations, LA-Attention can largely improve the precision of the prediction model,
% \textcolor{red}{enhance the predictive quality}
which constitutes the two-stage training and testing schemes, shown in Algorithm \ref{alg:semi-lazy-training}. 
% \zl{An illustrative example of LA-Attention can refer to Appendix \ref{sec:appendix:example}.}

\iffalse
\begin{algorithm}[]
    \caption{LA-Attention: Locality-Aware Attention}
    \label{alg:nn}
    \KwIn{Key-value pair$\left( {X}_{\left(N \times d\right)}, {Y}_0_{\left(N \times 1\right)} \right)$, query set $X^{query}$, the threshold $thres$ and the training/testing flag.}
  	\KwOut{Super-class samples  ${X'}_{\left(N' \times d\right)}  \left(,{Y'}_{\left(N' \times 1\right)}\right)$}
  	Init $select \; list = \mathcal{I}$ \\
    \For{$each \; point \; x \; \textbf{in} \; X^{query}$}{
        % Get the neighbors $\mathcal{N}(x)$ of $x$. \\  % using RNN/KNN methods. \\
        Estimate $\hat{p}_x = \sum_i y_i \frac{k(x_i, x)}{\sum_j k(x_j, x)}$ \quad $(x_i,y_i) \in (X,Y_0)   $ \\
        \If{$\hat{p}_x$ > thres}{
            \If{training flag}{$\mathcal{I} \cup \left\{\left(x, \text{\textit{get label}}(x)\right)\right\}$}
            \Else {$\mathcal{I} \cup \left\{\left(x\right)\right\}$}}
    }
    \textbf{if} \textit{training flag} \textbf{then Return:} ${X'}, {Y'}$ \\
    \textbf{else} \textbf{Return:} ${X'}$ \\
    % \Else {\textbf{Return:} ${X'}$}
\end{algorithm}
\fi

\subsubsection{Metric Learning Module}
\label{sec:metric}
\
\newline
\indent Many approaches in machine learning require a measure of the distance among data points. Traditionally, practitioners would choose a standard distance metric (Euclidean, City-Block, Cosine, etc.) using prior domain knowledge. 
Indeed, different investors have different understanding of the financial market and prefer completely different types of factors, \emph{e.g.,}  value investors prefer fundamental factors, while active investors focus on technical factors. 
% It results in a large divergence of the input features. 
In order to enhance the flexibility of LARA, we turn to the metric learning technique to mitigate the pressure of manually searching for the suitable distance measurement of different factors. LARA automatically learns a proper distance metric in a given feature space. 
We adopt the Sparse High-Dimensional Metric Learning~(SDML) algorithm, an efficient sparse metric learning technique in high-dimensional space via double regularization, introduced in \cite{qi2009efficient}, and equip it in LARA as shown in Fig. \ref{fig:framework}. Overall, we use the \emph{metric learning module} to learn a well-suited distance metric assisting the \emph{localization module} to extract potentially profitable samples.

% \subsection{Understanding Locality-Aware Attention in LARA}
% \label{sec:understanding}
% We propose the locality-aware attention algorithm. It extracts the potentially profitable samples by attending to label information and locally construct a more accurate classifier. Specifically, it divides the feature space of financial datasets into distinct regions according to the \emph{localization module} (Figure \ref{fig:framework}) and gets potentially profitable samples in the light of the results of \emph{locality-aware attention} (Sec. \ref{sec:attention}). 
% % As a consequence, 
% Therefore, a natural problem arises here: 
% \emph{Is locality-aware attention in LARA useful for extracting potentially profitable samples?}

% \begin{figure}[htbp]
% 	% \setlength{\belowcaptionskip}{-0.5cm}
% 	\centering
% 	\includegraphics[width=.40\textwidth]{pics/case-study.pdf}
% % 	\vspace{-0.85cm}
% 	\caption{The didactic example for illustrating Locality-Aware Attention. Sample 200 data points from $\mathcal{N}\left( \left(-2,2\right), 4I_2 \right)$ and $\mathcal{N}\left( \left(2,-2\right), 4I_2 \right)$ as positive and negative training samples, respectively. Testing samples are from the same distribution. The blue region (upper left) stands for the super-positive area with less noise. The same for the supeR-Neighboregative area in the red region (lower right). For a linear classifier $y = w \cdot x$, the red dotted line represents the optimal solution and other solutions deviate from the optimal one (mainly located in green) due to insufficient samples and noise.}
% 	\label{fig_case}
% \end{figure}

% We use a didactic example to study the above proposed question in Figure \ref{fig_case}. Even though the optimal linear classifier (omitting the bias term for convenience) is determined\footnote{This conclusion is intuitive, and the rigorous mathematical proof can refer to \cite{bishop2006pattern}.}, $y = x$ , to classify $\mathcal{N}\left( \left(-2,2\right), 4I_2 \right)$ and $\mathcal{N}\left( \left(2,-2\right), 4I_2 \right)$, the actual classifier built over the whole set deviates from the optimal classifier owing to the insufficient samples and noise, especially in the region where positive and negative samples are mixed together. Intuitively, extracting samples in the blue and red regions with less noise and then building classifiers over them can generate a more robust decision boundary around the optimal one. Moreover, in the testing phase, the blue and red region samples are more robust to the deviation of the decision boundary, which may fail in the green region.
% Hence, the \emph{locality-aware attention} algorithm, which focuses on samples in the blue and red region, is more robust to the deviation of the learned decision boundary and deserves further study.


\subsection{Adaptive Refined Labeling}
\label{sec:bi-level}

\begin{algorithm}[b]
    \caption{\fontsize{9.8pt}{9.8pt}\selectfont RA-Labeling: Adaptive \underline{R}efined L\underline{a}beling}
    \label{alg:Bi-level-label}
    \KwIn{Training data $\left(X, Y_0\right) \in \mathcal{R}^{N \times d} \times \mathcal{R}^{N}$, the initial model $f_{\theta_0}: \mathcal{R}^{N \times d} \rightarrow \mathcal{R}^{N}$, iteration number of adaptive refined labeling $k$, and exchange ratio $r$.}
  	\KwOut{$f_{\theta_{\left[k\right]}} \in \mathcal{R}^N$.}
  	Init $f_{\theta_0}$ trained on $(X,Y_0)$.\\
    \For{$i \; \textbf{in} \; range\left( k \right)$}{
        $\hat{p} = f_{\theta_i}(X)$. \\
        $\left(X, Y_{i+1}\right) =$ sort $\left(X, Y_i\right)$ according to $\hat{p}$ in descending order.\\
        Reset the first $\left(N \times r\right)$ labels in $Y_{i+1}$ to $1$. \\
        Reset the last $\left(N \times r\right)$ labels in $Y_{i+1}$ to $0$. \\
        % Get the index $\text{idx}_1$ with the $\left(N \times r\right)$ highest $\hat{p}$ and $\text{idx}_2$ with the $\left(N \times r\right)$ lowest $\hat{p}$. \\
        % Set $\hat{Y_1} = \left[0,\cdots,0\right] \in \mathcal{R}^N$; $\hat{Y_2} = \left[0,\cdots,0\right] \in \mathcal{R}^N$. \\
        % $\hat{Y_1}\left[\text{idx}_1\right] = 1$; $\hat{Y_2}\left[\text{idx}_2\right] = 1$. \\
        % $\hat{Y_1} =$ the label of top $r$ ratio samples with the highest $\hat{p}$. \\
        % $\hat{Y_2} =$ the label of bottom $r$ ratio samples with the lowest $\hat{p}$. \\
        % $Y_{i+1} = \left(Y_i \land \hat{Y_1}\right) \lor \left( \neg Y_i \land \hat{Y_2} \right)$.\\
        % $\hat{p}' = f_{\theta_{i}}(X)$ \\
        % $l = Loss\left(Y_{i+1}, \; \hat{p}'\right)$ \\
        % Retrain $f_{\theta_i}(X)$ according to $l$ to get $f_{\theta_{i+1}}(X)$\\
        Retrain $f_{\theta_i}$ according to $(X,Y_{i+1})$ to get $f_{\theta_{i+1}}$.\\
    }
    \textbf{Return:} $f_{\theta_{\left[k\right]}}$ = $Combine(\{f_{\theta_{i}}, 0 \leq i \leq k\})$. \\
\end{algorithm} 

Price movement is notoriously difficult to forecast because financial markets are complex dynamic systems~\cite{samuelson2016proof}.
% due to the highly stochastic and chaotic nature of financial markets \cite{samuelson2016proof}. 
% In addition, 
Indeed, we observe that some training samples get the high~(low) probability of the positive prediction $Pr(y=1)$, but their labels might also be negative~(positive). Thus, we name them as the \emph{noisy samples}.
% \textcolor{red}{This is an actual instance that a Bernoulli trial has sampled a negative (positive) label $y_{|x}$ even with high (low) $p_x$, recall that $y_{|x} \sim Ber(p_x)$ in our assumption. } 
% Recalling that $y_{|x} \sim Ber(p_x)$ in our assumption, we call them \emph{noisy samples} because a Bernoulli trial has sampled a negative (positive) label even with the high (low) $Pr(y=1)$.
% of one-time sampling of independent Bernoulli distribution.
% Recall that $y_{|x} \sim Ber(p_x)$ in our assumption, we consider that the over-confident negative samples have negative labels but get high $p_x$ because of one-time sampling. 
% \textcolor{red}{In consequence}, 
We propose to reset the labels of these \emph{noisy samples} to the opposite ones, \emph{i.e.,} positive training samples with the extremely low predicted probability are modified to the negative label,
% \textcolor{blue}{\sout{while those negative ones are modified to the positive}} 
and vice versa. 
Then we re-train another predictor based on the refined dataset with the modified labels.
In addition, our method runs in an iterative fashion. 
In each iteration of the training phase, it refines the labels of \emph{noisy samples} adaptively. 
In particular, denote the refined labels in the $i$-th iteration as $Y_i$. We sort training samples according to the probability of the positive prediction in descending order.
% and get $Y_{i+1}$. 
The process of refining positive samples to the negative can be described as resetting the last $\left(N \times r\right)$ labels in $Y_{i+1}$ to $0$, where $r$ is the exchange ratio taking the value from $[0,1]$. Meanwhile, the process of refining negative samples to the positive can be described as resetting the first $\left(N \times r\right)$ labels in $Y_{i+1}$ to $1$.
At last, we combine all the iterated predictors using the following proposed approaches:

\begin{itemize}[leftmargin=14pt]
\item \textbf{Last:} making a prediction from the last iterated predictor.
\item \textbf{Vote:} making a prediction that averages all iterated predictors.
% \item \textbf{and}:  making a prediction 
% % that is the and operation of
% at the consensus of multiple iterated predictors.
\end{itemize}

An illustration using the vote combining method is shown in Fig. \ref{fig_bi-level}. 
We can find that, in iteration 1, the weak learners can discriminate the vast majority of samples correctly, except for only one misclassified sample. In iteration 2, the algorithm further classifies all samples correctly after resetting two \emph{noisy samples'} labels adaptively and combining two more predictors.
This modification can be incorporated into existing machine learning codes easily: Add the $\left(4-6\right)$-th line in Algorithm \ref{alg:Bi-level-label} to refine the labels of the top and bottom $\left(N\times r\right)$ samples.
% More formally, RA-Labeling is depicted in Algorithm \ref{alg:Bi-level-label}. Despite the seemingly complex process of the RA-Labeling, we present a simple implementation for refined labels shown in the \textit{$6$-th} line of Algorithm \ref{alg:Bi-level-label}.
Finally, we combine all the trained models so far to boost the performance of predictors.

\begin{figure}[tbp]
	% \setlength{\belowcaptionskip}{-0.5cm}
	\centering
	\includegraphics[width=.4\textwidth]{pics/labeling.pdf}
	\vspace{-0.2cm}
	\caption{An illustration for the \emph{Adaptive Refined Labeling} method. The plus signs mean the positive samples and the minus signs mean the negative samples. The dot circle means resetting the label of samples to the opposite. The decision areas are represented in different colors~(Best viewed in color).}
	\label{fig_bi-level}
	\vspace{-0.4cm}
\end{figure}

% For a more intuitive comparison and to further understand the effectiveness of metric learning incorporated into the localization module, as shown in Fig. \ref{fig:tsne}, we plot the feature embedding of the sampled 1000 points of the test set using t-SNE \cite{van2008visualizing}.
% As mentioned above, we intend to search for as many \emph{super-positive} samples with $\hat{p}_x > 0.5$ as possible.
% In Fig. \ref{fig:tsne}(a), the positive and negative points in the original dataset are mixed together and there are 174 positive samples in total, which is hard to extract effectively. Using only the \emph{localization module} without \emph{metric learning} (Fig. \ref{fig:tsne}(b)), more positive samples (279) are found, indicating the effeteness of LA-Attention, but the negative ones still dominate. Further combined with \emph{metric learning}, in Fig. \ref{fig:tsne}(c), we can see the number of the positive samples (424) approximately halves in total. Hence, this learned distance metric can assist the \emph{locality-aware module} to further boost the estimation of \emph{super-class} samples.

% \begin{figure}[htbp]
% 	% \setlength{\belowcaptionskip}{-0.5cm}
% 	\centering
% 	\includegraphics[width=.48\textwidth]{pics/t-sne.pdf}
% 	\vspace{-0.4cm}
% 	\caption{Visualization for (a) Dataset (b) \emph{Super-positive} samples selected by the \emph{localization module} only (c) \emph{Super-positive} samples selected by LA-Attention.
% 	% (a) 5000 instances sampled from testing dataset for better visualization. (b) Instances uniformly sampled from (a) with the same number of as that in (c). (c) Super-class samples extracted by Label Attention equipped with Metric Learning. In above, \textcolor{yellow}{yellow} points stand for the positive and \textcolor{brown}{brown} points stand for the negative.
% 	}
% 	\label{fig:tsne}
% \end{figure}

\subsection{Implementation}
\label{sec:implementation}
As the \emph{localization module} needs to estimate attention weights to extract potentially profitable samples, a straightforward approach is to calculate the distance between all possible pairs of samples, which is computationally expensive when considering the quadratic explosion with respect to the number of datasets.
% To implement LA-Attention among the whole dataset, there are more than 0.4 million samples, so it is unrealistic to calculate the distance between each pair of them. 
We utilize our proposed \emph{masked attention} scheme to calculate attention weights located in the neighborhood of each sample, \textit{i.e.,} $\mathcal{N}(x)$.
However, it is still time-consuming to accurately search for the neighbors $\mathcal{N}(x)$ of the corresponding sample $x$. Then we adopt a fast approximate nearest neighbor search method called HNSW~\cite{malkov2018efficient}, and it provides more than 100 times speedup to approximately query the nearest neighbors.
In particular, we propose two schemes to obtain the neighbors of each sample based on the HNSW algorithm: the first is to search for the K-nearest neighbors (K-Neighbor) and the second is to search for the nearest neighbors in a fixed radius (R-Neighbor). 
The HNSW algorithm can be directly adopted in K-Neighbor. As for R-Neighbor, we first query the nearest neighbors with the moderate value of K and then select potentially profitable samples located in a fixed radius.
% Since we implement R-Neighbor based on HNSW, we have to first query k nearest neighbors and then select those located in a certain radius.
% Considering two kinds of attention weight: the first is identical weight $k_i$ and the second is the reciprocal of distance $k_r$. Then the attention to the labels from neighborhood $\mathcal{N}(x)$ can be formulated as follows:
% \begin{equation}
%     \label{eq:KNN-RNN-estimation-methods}
%     \begin{aligned}
%     \hat{p}_x &= \sum_{z \in \mathcal{N}(x)} y_z \frac{k(z, x)}{\sum_{z \in \mathcal{N}(x)} k(z, x)}, \quad k \in \{k_i, k_r\}
%     \end{aligned}
% \end{equation}
% \begin{equation}
%     \left \{
%     \begin{aligned}
%     k_i(z,x) & = 1 , \text{identical weight}\\
%     k_r(z,x) & = 1/d(z, x) , \text{the reciprocal of distance}
%     % k_i(z, x) &= 1 \\
%     % k_r(z, x) &= 1 / d(z, x)
%     \end{aligned}
%     \right.
%     ,
% \end{equation}
% where $d(., .)$ denotes Euclidean distance and $y_z$ denotes that actual label of datapoint $z$.
As introduced in Sec.~\ref{sec:attention}, we consider two kinds of attention weights: the identical weight $k_i$ to implement the K-Neighbor algorithm and the reciprocal of distance $k_r$ to implement the R-Neighbor algorithm.
% We apply $k_i$ to implement the K-Neighbor algorithm and apply $k_r$ to implement the R-Neighbor algorithm. 
The pseudocode for the K-Neighbor/R-Neighbor is detailed in Algorithm \ref{alg:KNN-RNN-algorithm}.
\begin{algorithm}
    \caption{K-Neighbor and R-Neighbor Algorithm}
    \label{alg:KNN-RNN-algorithm}
    \KwIn{Training data $\left(X, Y\right) \in \mathcal{R}^{N \times d} \times \mathcal{R}^{N}$, the query sample $x$, the number of the nearest neighbors $K$, and the radius $R$.}
  	\KwOut{$\hat{p}_x \in \mathcal{R}^N$.}
  	\nonl \textbf{K-Neighbor Algorithm: } \\
  	$\mathcal{N}(x)$ = top $K$ points with minimum $d(z, x)$, $z \in X$.\\
  	\textbf{Return:} $\hat{p}_x = \sum_{z \in \mathcal{N}(x)} y_z \frac{k_i(z, x)}{\sum_{z \in \mathcal{N}(x)} k_i(z, x)}$. \\
    % \textbf{Return:} $\hat{p}_x$\\
    
    \nonl \rule[10pt]{8.3cm}{0.05em}
    \textbf{R-Neighbor Algorithm: } \\
    \setcounter{AlgoLine}{0}
  	$\mathcal{N}_1(x)$ = top $K$ points with minimum $d(z, x)$, $z \in X$.\\
  	$\mathcal{N}_2(x)$ = $\{z: z \in \mathcal{N}_1(x),\; d(x, z) < R \}$. \\
  	\textbf{Return:} $\hat{p}_x = \sum_{z \in \mathcal{N}_2(x)} y_z \frac{k_r(z, x)}{\sum_{z \in \mathcal{N}_2(x)} k_r(z, x)}$. \\
    % \textbf{Return:} $\hat{p}_x$\\
\end{algorithm}

Algorithm \ref{alg:semi-lazy-training} describes the whole process of the LARA framework. As we study the binary classification problem, we use the binary cross-entropy loss in RA-Labeling. Note that the \emph{localization module} in LARA does not rely on specific methods as the backbone predictor. For the sake of simplicity, we use \emph{LightGBM}~\cite{ke2017lightgbm}, a commonly used GBDT open-sourced implementation, as the base predictor in our experiments. The RA-Labeling method can also be used in conjunction with the other machine learning algorithms to denoise the \emph{noisy samples} in quantitative trading. 
Thus, LARA is a versatile framework, and existing deep learning methods of price movement forecasting can be also integrated into the framework.
\begin{algorithm}[]
    \caption{LARA framework}
    \label{alg:semi-lazy-training}
    % \NoNumber{$\triangleright$ \textbf{Training phase: }} \\
    \KwIn{Training data $\left(X, Y\right) \in \mathcal{R}^{N \times d} \times \mathcal{R}^{N}$, testing data $X_{test} \in \mathcal{R}^{N_{\text{test}} \times d}$, the initial model $f_{\theta_0}$, threshold $thres$, hyper-parameters $k$, $r$.}
  	\KwOut{$Y_{out} \in \mathcal{R}^N$.}
%   	Init $f_{\theta_0}$ \\
  	$\vartriangleright$ \textbf{Training phase: } \\
  	Init \textit{emtpy set} $X', Y'$. \\
  	\For{$(x,y)$ \textbf{in} $(X, Y)$}{
  	    Estimate $\hat{p}_x$ via Eq. \eqref{eq:label-attention-reformulate} with the query sample $x$ and the key-value pair $(x_i, y_i) \in (X,Y)$.\\
  	    \textbf{if} {$\hat{p}_x$\textgreater  \text{thres}} \textbf{then} $X' \cup \{x\} ; \; Y' \cup \{y\}$. \\
  	}
  	$f_{\theta_{\left[k\right]}}$ = RA-Labeling $\left( {X'}, {Y'}, f_{\theta_0}, k, r\right)$. \\
  	$\vartriangleright$ \textbf{Testing phase: } \\
  	Init \textit{emtpy set} $X_{test}'$. \\
  	\For{$x_{\text{test}}$ \textbf{in} $X_{test}$}{
  	    Estimate $\hat{p}_{x_{\text{test}}}$ via Eq. \eqref{eq:label-attention-reformulate} with the query sample $x_{\text{test}}$ and the key-value pair $(x_i, y_i) \in (X,Y)$.\\
  	    \textbf{if} {$\hat{p}_x$\textgreater  \text{thres}} \textbf{then} $X_{test}' \cup \{x_{\text{test}}\}$. \\
  	}
  	\textbf{Return:} $Y_{out} = f_{\theta_{\left[k\right]}}(X_{test}')$. \\
\end{algorithm}

==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{sec:conclusion}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerNA{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See Section~\ref{sec:experiments} and supplementary materials}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Appendix~\ref{sec:appendix-B}}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{See results with error bars in Table~\ref{table:main} and \ref{table:imbalanced-type}}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Appendix~\ref{sec:appendix-B}}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See Section~\ref{sec:experiments}.}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

